AutoDIR: Automatic All-in-One Image Restoration with Latent Diffusion

We present AutoDIR, an innovative all-in-one image restoration system incorporating latent diffusion. AutoDIR excels in its ability to automatically identify and restore images suffering from a range of unknown degradations. AutoDIR offers intuitive open-vocabulary image editing, empowering users to customize and enhance images according to their preferences. Specifically, AutoDIR consists of two key stages: a Blind Image Quality Assessment (BIQA) stage based on a semantic-agnostic vision-language model which automatically detects unknown image degradations for input images, an All-in-One Image Restoration (AIR) stage utilizes structural-corrected latent diffusion which handles multiple types of image degradations. Extensive experimental evaluation demonstrates that AutoDIR outperforms state-of-the-art approaches for a wider range of image restoration tasks. The design of AutoDIR also enables flexible user control (via text prompt) and generalization to new tasks as a foundation model of image restoration. Project is available at: \url{https://jiangyitong.github.io/AutoDIR_webpage/}.

==> sec/method_old.tex <==
\begin{figure}[h!]
    \centering
    \includegraphics[width=\columnwidth]{figures/20231115_method.pdf}
    \vspace*{-6mm}    
    \caption{Diagram of the proposed Blind Image Quality Assessment (BIQA) module. Refer to Section~\ref{subsec:biqa} for more details.}
    \label{fig:framework}
\end{figure}

%-------------------------------------------------------------------
\vspace{-1em}
\section{Our Method}
\label{sec:method}
Figure~\ref{fig:representative} shows the overall flowchart of the proposed AutoDIR (Automatic All-in-One Image Restoration with Latent Diffusion), a unified model that can automatically detect and address multiple unknown degradations in images. AutoDIR consists of three parts:
% \vspace{6pt}
\begin{itemize}
    \item Semantic-Agnostic Blind Image Quality Assessment (BIQA): This module automatically identifies the predominant degradations present in the input image, such as noise, blur, haze, and generates a corresponding text prompt, denoted as $e_{auto}$, which is subsequently used in the image restoration process.
    % \vspace{5pt}
    \item  All-in-one Image Restoration (AIR): This module is based on a pre-trained latent diffusion model~\cite{rombach2022high}. With the guidance from the text embedding $e_{auto}$ from BIQA or user-provided open-vocabulary instruction $e_{user}$, the AIR module outputs a restored image  $I_{sd}$.   
    % \vspace{5pt}
    \item Structural-correction module (SCM): SCM is a lightweight convolution network that aims to further restore image details and correct remaining distortions in $I_{sd}$ in a residual manner. The output of this restoration process is the final restored image, denoted as $I_{res}$.
\end{itemize}


\subsection{Semantic-Agnostic Blind Image Quality Assessment (BIQA)}
\label{subsec:biqa}

 % We consider seven common distortions in images $ c \in \mathcal{C} = \{$ "noise", "blur", "rain", "underexposure", "haze", "low resolution", "raindrop" $\}$. 
%  As illustrated in Fig.~\ref{fig:framework}, 
% Let $\mathcal{C}$ denotes the set of image distortions, i.e. $ \mathcal{C} = \{c_{1}, c_{2}, ..., c_{K} \}$, where $c_{i}$ is an image distortion type, e.g. ``noise'' and $K$ is the number of distortions we consider.
%  The textural description prompt set is $\mathcal{T} = \{T $ $| T =$ “A photo needs $\{c_i\}$ artifact reduction.”, $c \in \mathcal{C}\}$.
% Given a corrupted image $I$ which undergoes several unknown artifacts, our BIQA aims to identify the dominant degradation of $I$ and extract the corresponding text embedding. 
%
We observe that classifying image degradation solely based on image information is challenging as shown in Sec.~\ref{sec:experiments}. We propose to leverage human language knowledge to enhance the detection of image degradation by employing a CLIP model~\cite{radford2021learning} as our Semantic-Agnostic BIQA backbone. we create a degradation description text prompts set and establish a connection between human language knowledge and image quality. However, since the pre-trained CLIP is pre-trained for visual recognition tasks emphasizing semantic information rather than image quality and has low accuracy in BIQA tasks.~\ref{sec:experiments}.
%
To overcome this, we tackle the problem in Two steps:
%%
(ii)We construct a new image quality assessment task for fine-tuning CLIP.
%
(iii) We propose a new regularization term for semantic-agnostic and image-quality-aware training.

As illustrated in Fig.~\ref{fig:framework}, 
let $\mathcal{C}$ denotes the set of image distortions, i.e. $ \mathcal{C} = \{c_{1}, c_{2}, ..., c_{K-1}, c_{K}\}$, where $c_{i}$ is an image distortion type, e.g. ``noise'' and $K-1$ is the number of distortions we consider. We also add a special type $c_{K}$ ="no" to indicate the end of the automatic multiple-step restoration.
 The textural description prompt set is $\mathcal{T} = \{T $ $| T =$ “A photo needs $\{c_i\}$ artifact reduction.”, $c \in \mathcal{C}\}$. 
Given a corrupted image $I$ which undergoes several unknown artifacts, our BIQA aims to identify the dominant degradation of $I$ and extract the corresponding text embedding. 
BIQA consists of an image encoder $\mathcal{E_I}$
and a text encoder $\mathcal{E_T}$. We first obtain the image embedding $\mathcal{E_I}( I) \in \mathbb{R}^d $ and the text embedding $\mathcal{E_T}(T) \in \mathbb{R}^{K \times d}$, then we compute the cosine similarity between image embedding $\mathcal{E_I}( I)$ and each prompt embedding $\mathcal{E_T}(T_i) \in \mathbb{R}^d $ by:
\begin{equation}\label{eq:logits}
     \textrm{logit}(c_i | I) =  \frac {\mathcal{E_I}( I) \cdot \mathcal{E_T}(T_i)}{ \|\mathcal{E_I}( I)\|_2 \| \mathcal{E_T}( T_i)\|_2 },
     % \mathbf{I_c} = \mathbf{I_n} + \sum_{i=1}^{L}\bar{c}_i \tilde{\mathcal{N}}_i, 
\end{equation}
where $T_i$ is the $i$-{th} element of $ \mathcal{T}$. Next, we calculate the probability $\hat{p}(c_i | I)$ and obtain the output text embedding of BIQA ${e}_{auto}$ by:  
\begin{equation}\label{eq:probability}
\hat{p}(c_i | I) = \frac{\exp(\textrm{logit}(c_i | I))}{\sum_{i=1}^{K} \exp(\textrm{logit}(c_i | I))},
\end{equation}
\begin{equation}\label{eq:textout}
{e}_{auto} = \sum_{i=1}^{K} \hat{p}(c_i | I)  \mathcal{E_T}( T_i).
\end{equation}
\paragraph{\textbf{Naive fine-tuning on image quality assessment}}
During the optimization of BIQA, we freeze the parameters of the text encoder $\mathcal{E_T}$ and finetune the image encoder $\mathcal{E_I}$ using the multi-class fidelity loss \cite{tsai2007frank}. The fidelity loss can be denoted as:
% \begin{equation}\label{eq:cliploss}
% L_{FID} = 1 - \sum_{i=1}^{K} \sqrt{p(c_i| I)\hat{p}(c_i| I)},
% \end{equation}
\begin{equation}\label{eq:cliploss}
L_{FID} = 1 - \sum_{i=1}^{K} \sqrt{y(c_i| I) \hat{p}(c_i| I)},
\end{equation}
% where $p(c_i| I)$ is a binary variable that equals 1 if $c_i$ is the dominant degradation in image $I$, and 0 otherwise.
where $y(c_i| I)$ is a binary variable that equals 1 if $c_i$ is the dominant degradation in image $I$, and 0 otherwise. 
\paragraph{\textbf{Semantic-Agnostic Constraint fine-tuning on image quality assessment}}

% To support user-defined prompts, we use fine-tuned $\mathcal{E_T}$ to extract text embedding $\hat{e}_{user}$.

% During training, we freeze the parameter in $\mathcal{E_T}$ and use the multi-class fidelity loss \cite{tsai2007frank} to finetune the image encoder $\mathcal{E_I}$:
% \begin{equation}\label{eq:cliploss}
%  L_{BIQA} = (1-\sum_{i=1}^{V} \sqrt{p(c_i| I)\hat{p}(c_i| I)})
% \end{equation}
% where $p(c_i| I)$ =1 if $c_i$ is the dominate artifact of $I$. 

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/20231025_tsneclip.pdf}
    \vspace{-1em}
    \caption{t-SNE visualization of image embeddings  $\mathcal{E_I}( I)$ of CLIP of Blind Image Quality Assessment (BIQA) on SOTs dehazing dataset \cite{li2018benchmarking}. Image embeddings of foggy images and their ground-truth clean images are extracted by a) original CLIP. b) finetuned CLIP. c) CLIP finetuned with semantic-agnostic constraint. This illustrates that semantic-agnostic constraint can separate the embeddings of the degraded images from the clean images, while original CLIP and finetuned CLIP features cannot.}
    \vspace{-1em}
    \label{fig:clip_ab}
\end{figure}

% In the pre-trained CLIP model,  designed for image classification, primarily emphasizes semantic information rather than image quality. During finetuning on image quality tasks, it is observed that the CLIP model tends to differentiate images based on semantic content. To address this issue, we propose the inclusion of a straightforward yet essential constraint to prevent the model from relying solely on semantic information but the image quality when classifying image degradation.

Since the original CLIP model is pre-trained on tasks such as image classification, its corresponding $\mathcal{E_I}(I)$ encoders tend to encode images based on their semantic information (\eg, cat or dog) rather than their image quality (\eg, noisy or clean). When we fine-tune the CLIP model for generating texts for BIQA according to image quality, this becomes a significant limitation. 
As shown in Fig.~\ref{fig:clip_ab} a) and b), the image embeddings extracted by the original CLIP and the finetuned CLIP on foggy, as well as their corresponding ground-truth clean images, cannot be separated, indicating a focus on semantic information rather than image quality differences.

To address this issue, we propose a novel approach called the semantic-agnostic constraint loss ($L_{SA}$) to regulate the fine-tuning process and prevent the model from relying solely on semantic information rather than image quality. 
The semantic-agnostic loss ($L_{SA}$) applies a penalty when the CLIP model suggests that the artifact $c_i$ is present in the ground-truth clean image  $I_{gt}$ which corresponds to the degraded image $I$. This penalty forces the BIQA model to distinguish between $I_{gt}$ and $I$ based on image quality, encouraging the CLIP image encoder ($\mathcal{E_I}(I)$) to focus on extracting image quality information rather than semantic information.
This constraint loss can be derived using the following equation:
\begin{equation}\label{eq:cliploss}
L_{SA} = \sum_{i=1}^{K} \sqrt{y(c_i|I)\hat{p}(c_i| I_{gt})},
\end{equation}
where $y(c_i|I)$ is a binary variable that is equal to 1 if $c_i$ represents the dominant degradation in image $I$, and 0 otherwise, and $\hat{p}(c_i|I_{gt})$ denotes the probability that the dominant degradation in $I_{gt}$ is represented by $c_i$.
%
% The semantic-agnostic loss ($L_{SA}$) applies a penalty when the CLIP model suggests that the artifact $c_i$ is present in the ground-truth image $I_{gt}$. This penalty forces the BIQA model to distinguish between $I_{gt}$ and $I$ based on image quality, encouraging the CLIP image encoder ($\mathcal{E_I}(I)$) to focus on extracting image quality information rather than semantic information.

We incorporate the semantic-agnostic constraint $L_{SA}$ with the fidelity loss $L_{FID}$, resulting in the total loss $L_{BIQA}$ for BIQA module:
%
\begin{equation}\label{eq:cliploss_total}
L_{BIQA} =  L_{FID} + \lambda L_{SA},
\end{equation}
where we set $\lambda=1$ in our experiments.
% The effectiveness of this constraint is further verified in Section \ref{sec:analysis}.
As shown in Fig.~\ref{fig:clip_ab} c), CLIP fine-tuned with a semantic-agnostic constraint can separate the embeddings of the degraded images from the clean images as expected. 

% In Figure \ref{fig:clip_ab}, we evaluate the ability of our BIQA model to cluster embeddings based on the specific artifact itself, e.g. haze degradation in Synthetic Objective Testing Set (SOTs)~\cite{li2018benchmarking} dehazing dataset, rather than the content differences across different datasets.
% Such behavior has been observed to be associated with finetuning with the Semantic-agnostic constraint. 
% Specifically, before and after finetuning without Semantic-agnostic constraint, the feature extracted from degraded images cannot be distinguished from clean images, indicating a focus on the semantic information. 
% %
% However, after our finetuning without Semantic-agnostic constraint, the degraded image embeddings can be separated from the clean image embeddings, showing improved artifact detection.
% The output text embedding of BIQA is:
% \begin{equation}\label{eq:cliploss}
% \hat{e}_{auto} = \sum_{i=1}^{V} \hat{p}(T_i | I)  \mathcal{E_T}( T_i)
% \end{equation}

% Besides the automatic text embedding generated by the BIQA module, we also support user-defined prompts. Given a user instruction $\mathcal{P}$, we extract the text embedding $\hat{e}_{user} = \mathcal{E}_T(\mathcal{P})$ as the guidance of the following image restoration module.
% % To support user-defined prompts, we use fine-tuned $\mathcal{E_T}$ to extract text embedding $\hat{e}_{user}$.
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/20231101_tsnemove.pdf}
    \vspace{-1em}
    \caption{t-SNE visualization of image embeddings $\mathcal{E_I}( I)$ with seven types of degradations, which illustrates the space of common image degradations. Images captured by Under-Display Cameras (UDC)~\cite{zhou2021image} suffer from both blur and underexposure. AutoDIR automatically decides (via BIQA) the first step is to improve "underexposure", and the second step is to remove "blur", moving the input images towards the region of clean images.}  
    %is first distributed in the underexposure area. After step-one editing, it shifts to the blurred artifact area, which indicates that the underexposure artifact is removed. After step-two deblurring editing, the embedding moves toward the clean image area.
    % t-SNE visualization of image embeddings on images with seven degradation types, unseen Under-Display Camera (UDC) dataset TOLED \cite{zhou2021image} and unseen Enhancing Underwater Visual Perception (EUVP) dataset \cite{islam2020fast}.} Embeddings of UDC input images, which contain blur and underexposure artifacts, are distributed between blur and underexposure areas. After step-one editing, they shift to the blurred artifact area, which indicates that the underexposure artifact is removed. Embeddings of EUVP dataset input images are distributed in the blurred artifact area and move to the haze area after the deblurring operation, which indicates that the blur artifact is removed and the haze artifact is the remaining dominant degradation.}
    \label{fig:tsne_move}
    \vspace{-.5em}
\end{figure}

\subsection{All-in-one Image Restoration (AIR)}
% In addition to the automatic text embedding generated by the BIQA module (${e}_{auto}$), AutoDIR also supports user-defined prompts for customized control. Given a user instruction $\mathcal{P}$, we can also extract the text embedding $e_{user} = \mathcal{E}_\mathcal{T}(\mathcal{P})$ as additional guidance for image restoration.
The All-in-one Image Restoration (AIR) module is designed to apply various operators for image restoration. Previous studies~\cite{wang2023stableSR,} have shown that generative models have a remarkable ability to generate missing or distorted details in image restoration, outperforming discriminative methods. Our observations in Section~\ref{sec:experiments} align with these findings, as we noticed that discriminative methods face challenges in demanding image restoration tasks such as super-resolution.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/20231116_crossatten.pdf}
    \caption{Cross-attention maps of text-conditioned diffusion image restoration. The top-left shows an input image with raindrops on the left half. The remaining plots show the cross-attention masks for the keywords “haze”, "low-resolution" and “raindrop” in the text prompt used for restoration. While the cross-attention maps for "haze" and "low-resolution" are more uniformly distributed over the entire image, the map for "raindrop" correctly focuses on the actual image artifacts, as expected.} 
    \label{fig:cross_att}
    \vspace{-1em}
\end{figure}

Therefore, we conduct the AIR module based on the generative model Latent Diffusion Model~\cite{rombach2022high}. AIR module utilizing both text and image embedding conditions to restore images $I_{sd}$ with generative priors. The text embedding condition, denoted as $e = \{ e_{auto}, e_{user} \}$, aims to disentangle different types of image degradations, while the latent image embedding condition $z_I = \mathcal{E}_{ldm}(I)$ from the image encoder $\mathcal{E}_{ldm}$ of the latent diffusion model~\cite{rombach2022high} is to provide information of image structures. To enable the text condition to guide different image restoration, we incorporate cross-attention~\cite{vaswani2017attention} to map the text condition $e$ into the intermediate layers of the time-conditional UNet backbone \cite{ronneberger2015u} of the Latent Diffusion Model~\cite{rombach2022high}.

%
For the image condition, we concatenate the image condition $z_I$ with the noisy latent $z_t$ and feed them to the UNet backbone. Consequently, the denoiser expression of the UNet backbone becomes $\epsilon_{\theta}(e, [z_t, z_I], t)$, where [~] denotes concatenation.
%
After the reversing process, we obtain the restored image $I_{sd}$ by passing the updated latent $\hat{z}$ through the decoder $\mathcal{D}$ of the Latent Diffusion Model, defined as $I_{sd} = \mathcal{D}(\hat{z})$.
%


\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/20231101_SCM.pdf}
    \caption{The Structural-Correction Module (SCM) is an additional convolution network to further improve image structures and details. As shown, image structures, i.e., human face and text, are severely distorted without SCM and recovered well with SCM.}
    \label{fig:SCM}
    \vspace{-1em} 
\end{figure}

\textbf{\paragraph{}}
While the latent-diffusion-based generative modes can hallucinate texture details, they sometimes struggle to maintain fine image structures such as human faces and texts as shown in Fig.~\ref{fig:SCM}. To address the structure distortion, we employ an efficient structural-correction module (SCM) denoted as $\mathcal{F}$. The purpose of SCM is to extract the contextual information $\mathcal{R}$ from the original image and incorporate it with the intermediate image restoration result $I_{sd}$ in a residual manner. This is achieved through the following equation:
%
\begin{equation}\label{eq:CBRMR}
I_{res} = I_{sd} + w \cdot \mathcal{F}( [ I_{sd}, I] ),
\end{equation}
%
where $[~]$ denotes concatenation, and $w$ is an adjustable coefficient that ranges between 0 and 1. The value of $w$ determines the extent to which contextual information is utilized to recover the final result. A larger value of $w$ emphasizes the use of contextual information, which is beneficial for tasks that require structure consistency, such as low light enhancement. Conversely, a smaller value of $w$ is often employed to maintain the generation capability of AIR for tasks like super-resolution. By integrating SCM, AutoDIR effectively restores the distorted context of the original image, seamlessly incorporating the enhancements made during the editing phase as shown in Fig.~\ref{fig:SCM}. 
%For more results, please refer to Section \ref{sec:ablation}.
\textbf{\paragraph{AIR training loss}}
During training, we fine-tune the UNet backbone $\epsilon_{\theta}(e, [z_t, z_I], t)$ for image restoration tasks. The objective function is defined as:
\begin{equation}\label{eq:OCLDM}
L_{AIR} =  \mathbb{E}_{\mathcal{E}_{ldm}(x), c_{I},e,\epsilon ,t} [\| \epsilon - \epsilon_{\theta}(e, [z_t, z_I] , t)\|_2^2].
\end{equation}
For the strutural correction, instead of sampling the  edited latent $\hat{z}_t$, which is time-consuming, we utilize the estimated edited latent $\Tilde{z}$, which is calculated by:
\begin{equation}
\Tilde{z} = \frac{z_t}{\sqrt{\bar{\alpha}}} - \frac{\sqrt{1-\bar{\alpha}} \epsilon_{\theta}(e, [z_t, z_I] , t)}{\sqrt{\bar{\alpha}}},
\end{equation}
where $\bar{\alpha}$ represents the noise scheduler introduced in \cite{rombach2022high}. The loss function for SCM is further defined as:
\begin{equation}
L_{SCM} = \| I_{gt} - \left(\mathcal{F}(\mathcal{D}(\Tilde{z}), I) + \mathcal{D}(\Tilde{z})\right)\|_2^2
\end{equation}


Fig.~\ref{fig:cross_att} shows our experiment of exploring the mechanism of the text conditions disentangling different image restoration tasks
% that different text conditions can yield corresponding different cross-attention maps 
during the reverse diffusion process.
We find that different text conditions yield different cross-attention maps. 
%which will further alternate the sampling results. 
As shown in Fig.\ref{fig:cross_att}, changing the text prompt leads
to significant changes in the cross-attention map. The map closely aligns with the text prompt, which either uniformly distributes attention across the entire image for the “dehazing” prompt, or concentrates on the part with edges or textures for the "low-resolution" prompt, or focuses on specific areas such as raindrops for the ``deraindrop'' prompt.
This shows that BIQA and AIR can guide the diffusion attention toward regions that are more likely to have image artifacts.
  
% \subsection{Training of AutoDIR.}
%  \vspace{-0.1cm} 
% The three components of AutoDIR are optimized using their respective objectives. 
% During the optimization of BIQA, we freeze the parameters of the text encoder $\mathcal{E_T}$ and finetune the image encoder $\mathcal{E_I}$ using the multi-class fidelity loss \cite{tsai2007frank}. The fidelity loss can be denoted as:
% %
% \begin{equation}\label{eq:cliploss}
% L_{FID} = 1 - \sum_{i=1}^{K} \sqrt{p(c_i| I)\hat{p}(c_i| I)}.
% \end{equation}
% %
% Here, $p(c_i| I)$ is a binary variable that equals 1 if $c_i$ is the dominant artifact in image $I$, and 0 otherwise.
%
% To encourage the CLIP model to focus on image quality, we incorporate the "Semantic-Agnostic" regularization $L_{SA}$, resulting in the total loss $L_{BIQA}$:
% %
% \begin{equation}\label{eq:cliploss_total}
% L_{BIQA} = L_{FID} + L_{SA}.
% \end{equation}

% For the AIR model, we fine-tune the UNet backbone $\epsilon_{\theta}(e, [z_t, z_I], t)$ for image restoration tasks. The objective function is defined as:
% %
% \begin{equation}\label{eq:OCLDM}
% L_{AIR} =  \mathbb{E}_{\mathcal{E}_{ldm}(x), c_{I},\hat{e},\epsilon ,t} [\| \epsilon - \epsilon_{\theta}(e, [z_t, z_I] , t)\|_2^2],
% \end{equation}
% where $[.]$  is concatenation operation.

% When training SCM, instead of sampling the  edited latent $\hat{z}_t$, which is time-consuming, we utilize the estimated edited latent $\Tilde{z}$, which is calculated by:
% \begin{equation}
% \Tilde{z} = \frac{z_t}{\sqrt{\bar{\alpha}}} - \frac{\sqrt{1-\bar{\alpha}} \epsilon_{\theta}(e, [z_t, z_I] , t)}{\sqrt{\bar{\alpha}}}.
% \end{equation}
% Here, $\bar{\alpha}$ represents the noise scheduler introduced in \cite{rombach2022high}. The loss function for SCM is further defined as:
% \begin{equation}
% L_{SCM} = \| I_{gt} - \left(\mathcal{F}(\mathcal{D}(\Tilde{z}), I) + \mathcal{D}(\Tilde{z})\right)\|_2^2
% \end{equation}

% \begin{algorithm}
% \caption{Training of SCM}\label{training_SCM}
% \begin{algorithmic}[1]
% \Repeat
% \State $x_0 \sim \mathcal{N}(0,1)$ \
% \Until{Converged}
% \end{algorithmic}
% \end{algorithm}




% The whole AutoDIR framework is end-to-end trained by jointly optimizing the three parts, where the final objective function is:
% \begin{equation}
%     L =  \lambda_{1} L_{BIQA} + \lambda_{2} L_{AIR} + \lambda_{1} L_{SCM}
% \end{equation},
% where  $\lambda_{i}, i=1,2,3$ is loss weights. 



% Convolutional-Based Restoration Module, utilizing a CNN-base network $\mathcal{F}$,  takes both the $I_{sd}$ and original image $I$ as input and output the final result:
% \begin{equation}\label{eq:finalres}
% \hat{I}_{res} = \mathcal{F}{(Concat(I_{sd}, I))} + I_{sd}
% \end{equation}

